Temporal Representation Learning on Monocular Videos for 3D Human Pose Estimation

In this paper we propose an unsupervised feature extraction method to capture temporal information on monocular videos, where we detect and encode subject of interest in each frame and leverage contrastive self-supervised (CSS) learning to extract rich latent vectors. Instead of simply treating the latent features of nearby frames as positive pairs and those of temporally-distant ones as negative pairs as in other CSS approaches, we explicitly disentangle each latent vector into a time-variant component and a time-invariant one. We then show that applying contrastive loss only to the time-variant features and encouraging a gradual transition on them between nearby and away frames while also reconstructing the input, extract rich temporal features, well-suited for human pose estimation. Our approach reduces error by about 50% compared to the standard CSS strategies, outperforms other unsupervised single-view methods and matches the performance of multi-view techniques. When 2D pose is available, our approach can extract even richer latent features and improve the 3D pose estimation accuracy, outperforming other state-of-the-art weakly supervised methods.

==> figures/ski_bg_base.tex <==
% !TEX root = ../cvpr.tex
% !TEX spellcheck = en-US

\begin{figure*}[!htb]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/bg1.jpg}
	\includegraphics[width=0.47\textwidth, height=3.05cm]{figures/bg2.jpg}
	\caption{\small {\bf Ski dataset background samples.} Two samples of estimated ski backgrounds are shown.}
	%The mask and the bbox location are learned by model without supervision through input image reconsuction. The parameters of the four sampled frames are shared.}
	\label{fig:ski_bg}
\end{figure*}


==> figures/supp_dive_pose4.tex <==
% !TEX root = ../cvpr.tex
% !TEX spellcheck = en-US

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{figures/supp_dive_pose4_fig.pdf}
	\caption{\small {\bf Qualitative results on Diving Dataset}.  	
	Samples are taken from the test set. In the top row, the red  rectangle shows the bounding box detected by our model for image cropping. The second and third rows, show respectively the decoded mask and re-synthesized image. Bottom rows show the pose estimation of our approach and the GT labels.}
	\label{fig:supp_dive_pose4}
	\vspace{1cm}
\end{figure*}


==> figures/supp_dive_pose5.tex <==
% !TEX root = ../cvpr.tex
% !TEX spellcheck = en-US

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{figures/supp_dive_pose5_fig.pdf}
	\caption{\small {\bf Qualitative results on Diving Dataset}.  
		Samples are taken from the test set. In the top row, the red  rectangle shows the bounding box detected by our model for image cropping. The second and third rows, show respectively the decoded mask and re-synthesized image. Bottom rows show the pose estimation of our approach and the GT labels.
	}
	\label{fig:supp_dive_pose5}
	\vspace{1cm}
\end{figure*}


==> tables/h36_2D_orig.tex <==
% !TEX root = ../cvpr.tex
% !TEX spellcheck = en-US

\begin{table}[ht]
	\centering
	\resizebox{.5\linewidth}{!}{
	\begin{tabular}{|l|c|}
		\hline
		\textbf{Model} & \textbf{\%-MSE Normalized Error} \\ \hline
		Thewlis et al.~\cite{thewlis19} & 7.51 \\
		Zhang et al.~\cite{Zhang18b} & 4.14 \\
		Lorenz et al. ~\cite{lorenz19} & 2.79 \\ 
		Jakab et al.~\cite{jakab20} & 2.73 \\
		Ours & \textbf{2.53} \\
		\hline
	\end{tabular}
}
\caption{\small {\bf Comparison against state-of-the-art 2D keypoint estimation models on H36M dataset.} \%-MSE normalized by image size is reported. All models predict 32 keypoints on 6 actions of wait, pose, greet, direct, discuss, and walk.}
\label{tab:h36_2D}
\end{table}


==> tables/merged.tex <==
% !TEX root = ../cvpr.tex
% !TEX spellcheck = en-US

\begin{table*}[ht]
\parbox{.75\linewidth}{
	\centering
	  \resizebox{1\linewidth}{!}{
		\begin{tabular}{|l|c|c|c|c|ccccc|}
			\hline
				\multirow{2}{*}{\textbf{Model}} &
			\multirow{2}{*}{\textbf{Decodes?}} & \multirow{2}{*}{\textbf{uses STN?}} & \multirow{2}{*}{\textbf{contrastive loss}} & \multirow{2}{*}{\textbf{latent split?}} &  \multicolumn{5}{c|}{\textbf{Percentage of Labeled Pose Data}} \\
			& & &  & & \textbf{0.3\% (100)} & \textbf{1\% (500)} & \textbf{14\% (5K)} & \textbf{50\% (17K)} & \textbf{all (35K)}\\
			\hline
			DSL & \color{red}{\xmark} & \color{red}{\xmark} &  DSL & \color{red}{\xmark} & 227.24 &  220.64 & 198.34 & 193.08 & 191.21 \\
			
			DSL-STN& \color{red}{\xmark} & \color{green}{\cmark} &  DSL & \color{red}{\xmark} & 236.32 & 211.85 & 202.57 & 199.16 & 198.22 \\
			
			 DSL-STN-Dec & \color{green}{\cmark} & \color{green}{\cmark} &  DSL & \color{red}{\xmark} &  185.75 & 159.34 & 135.93 & 129.62 & 127.52 \\
			
			AE-STN-Dec & \color{green}{\cmark} & \color{green}{\cmark} & \textemdash & \textemdash & 187. 25 & 161.53 & 130.21 & 117.044 & 114.73 \\

			CSS-STN-Dec-Split & \color{green}{\cmark} & \color{green}{\cmark} &  CSS & \color{green}{\cmark} & 163.61 & 137.52&  110.61 & 104.23 & 99.32 \\
			
			Ours & \color{green}{\cmark} & \color{green}{\cmark} &  DSL & \color{green}{\cmark} &  \textbf{149.32} &  \textbf{122.44} &  \textbf{100.23} &  \textbf{97.38} & \textbf{95.39} \\
			\hline
		\end{tabular}
	}
	\caption{\textbf{Ablation Study.} The last row shows our full model with all features applied. In the first two rows we apply the DSL contrastive loss without decoding and latent split. In the third row, we keep all the features except we do not split the latent components. In the fourth row, we apply only detection and reconstruction without any application of contrastive loss. In the fifth row, we only change the contrastive loss of our full model from DSL to CSS. In all settings, we observe a performance drop, however, the models without decoding suffer the most.}
	\label{tab:ablation}
}
\hfill
\parbox{.23\linewidth}{
	\centering
	\resizebox{1\linewidth}{!}{
		\begin{tabular}{|l|c|}
	\hline
	Model & 2D keypoint error \\ \hline
	Thewlis et al.~\cite{thewlis19} & 7.51 \\
	Zhang et al.~\cite{Zhang18b} & 4.14 \\
	Lorenz et al. ~\cite{lorenz19} & 2.79 \\ 
	Jakab et al.~\cite{jakab20} & 2.73 \\
	Ours & \textbf{2.53} \\
	\hline
\end{tabular}
}
\caption{\small {\bf Comparison against state-of-the-art 2D models on H36M dataset.} \%-MSE normalized by image size is reported. All models predict 32 keypoints on 6 actions of wait, pose, greet, direct, discuss, and walk.}
\label{tab:h36_2D}
}
\end{table*}

